Near-Optimal Schedules for Simultaneous Multicasts

We study the store-and-forward packet routing problem for simultaneous multicasts, in which multiple packets have to be forwarded along given trees as fast as possible. This is a natural generalization of the seminal work of Leighton, Maggs and Rao, which solved this problem for unicasts, i.e. the case where all trees are paths. They showed the existence of asymptotically optimal $O(C + D)$-length schedules, where the congestion $C$ is the maximum number of packets sent over an edge and the dilation $D$ is the maximum depth of a tree. This improves over the trivial $O(CD)$ length schedules. We prove a lower bound for multicasts, which shows that there do not always exist schedules of non-trivial length, $o(CD)$. On the positive side, we construct $O(C+D+\log^2 n)$-length schedules in any $n$-node network. These schedules are near-optimal, since our lower bound shows that this length cannot be improved to $O(C+D) + o(\log n)$.

==> optimal-routing.tex <==
\section{Near-Optimal Multicast Routing}
Here we note that our approach yields near-optimal multicast routing protocols for any graph and multicast requests. Specifically, if the optimal multicast routing protocol for a particular instance terminates in $T^*$ rounds, we obtain a routing protocol for the same instance terminating in $O(T^* + \log^2n)$ time.

\begin{thm}
	There exists a polynomial-time randomized algorithm $\mathcal{A}$ which for any multiple multicast instance with optimal scheduling time $T^*$, outputs a schedule of length $O(T^*+ \log^2n)$ with high probability.
\end{thm}
\begin{proof}
	A schedule which completes in $T$ rounds must in particular route the information along trees of depth at most $T$ from each sender to its group, such that each edge belongs to at most $T$ such trees. That is, if we denote by $\mcT_i(T)$ all trees of depth at most $T$ rooted at $s_i$ which span all of $S_i$, if we have an indicator variable $x_t$ for each tree in some $\mcT_i(T)$, we have 
	two constraints. The first is that each multicast session is satisfied, 
	\begin{equation}\label{constraint:span}
		\sum_{t\in \mcT_i} x_t \geq 1 \qquad \forall i\in [k],
	\end{equation}
	while the congestion constraints can be succinctly written as
	\begin{equation}\label{constraint:congestion}
		\sum_{t\ni e} x_t \leq T \qquad \forall e\in E.
	\end{equation}
	Relaxing the integrality requirement for the $x_t$ variables yields a polytope which can be solved efficiently, as its dual is approximately separable. 
	For example, if we try and optimize the trivial objective $0$ subject to constraints \eqref{constraint:span} and \eqref{constraint:congestion}, the dual LP has as its objective $\min \sum_e \ell_e \cdot T - \sum_i w_i$, subject to 
	\begin{equation}
		\sum_{e\in t} \ell_e \geq w_i \qquad \forall i\in [k],\,t\in \mcT_i(T),
	\end{equation}
	and the latter constraints can be verified efficiently. NOT, IT CANNOT.
\end{proof}


We note that the additive loss from the rounding itself is tight. Moreover, by our lower bounds for fixed trees of congestion $c$ and $d$ (sufficiently small) one cannot avoid the loss of an additive $\log n$ term  compared to the optimal congestion+dilation bound. As such, improving the rounding of this LP, as was done by Srinivasan and Teo \cite{srinivasan2001constant}, is in some sense unnecessary. (Check to see who worked on such improvements, if at all)

==> prelims.tex <==
\subsection{Formal Definition of \SM and Unicast}\label{sec:model}
We now formally define \sm and unicast and the notation we use throughout this work.

In the store-and-forward model, a network is modeled as a graph $G = (V, E)$. Time proceeds in discrete, synchronous rounds during which nodes trade atomic packets. In each round a node can send a packet it holds to any one of its neighbors, but at most one packet is allowed to be sent along an edge in each round. Nodes can copy packets and send duplicate packets to neighbors, again subject to the constraint that at most one packet crosses an edge each round. We assume that nodes can copy and broadcast packets as this is true for routers in standard IP multicast \cite{deering1988host}.

A \sm instance is given by a set of rooted trees $\mcT$ on a single store-and-forward graph $G$ where each $T_i$ has root $r_i$ and leaves $L_i$. Each $i$ also has associated with it a packet (a.k.a.\ message) $m_i$, initially only known to $r_i$. 
The congestion $C$ is defined as $\max_e |\{T_i \ni e\}|$ and the dilation $D$ is defined as $\max_i \text{depth}(T_i)$. 
A schedule instructs nodes what packets to send in which rounds, subject to the constraint that $m_i$ can only be sent over edges in $T_i$.
The quality of a schedule is its \emph{length}; i.e., the number of rounds until all nodes in $L_i$ have received $m_i$ for every $i$.
A \su instance is the simple case of a \sm where all $T_i$ are paths.
